Event-aided Direct Sparse Odometry

We introduce EDS, a direct monocular visual odometry using events and frames. Our algorithm leverages the event generation model to track the camera motion in the blind time between frames. The method formulates a direct probabilistic approach of observed brightness increments. Per-pixel brightness increments are predicted using a sparse number of selected 3D points and are compared to the events via the brightness increment error to estimate camera motion. The method recovers a semi-dense 3D map using photometric bundle adjustment. EDS is the first method to perform 6-DOF VO using events and frames with a direct approach. By design, it overcomes the problem of changing appearance in indirect methods. We also show that, for a target error performance, EDS can work at lower frame rates than state-of-the-art frame-based VO solutions. This opens the door to low-power motion-tracking applications where frames are sparingly triggered "on demand" and our method tracks the motion in between. We release code and datasets to the public.

==> figs/eds_fps_study_rebuttal.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[trim={.2cm 0 1.3cm 1.2cm},clip,width=.8\linewidth]{imgs/eds_dso_fps_study_with_orb_slam.pdf}
    \vspace{-2ex}
    \caption{Average Absolute Trajectory Error (RMS) in the dataset~[49] for ORB-SLAM [33], ORB-SLAM$^\ast$~(w/o loop closure), DSO~[4], DSO$^\ast$~(w/o recovery-tracking) and EDS~(ours).
    Errors are computed for EDS every time an event-frame is tracked (equal at any frame rate), whereas for the baseline frame-based methods they are computed only when a frame is received (i.e., according to the frame rate).
    }
    \label{fig:fps_study_rebuttal}
    \vspace{-3ex}
\end{figure}


==> tables/tab_compare_rot_events_and_frames.tex <==
\begin{table}[h]
\vspace{-1ex}
\centering
\begin{adjustbox}{max width=\linewidth}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llcccc}
    & & ESVO [26] %
    & USLAM [23] %
    & EVO [10] %
    & EDS (\textbf{Ours})\\
    & \textbf{Input} & E+E & E+F+I & E & E+F\\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Sequence}}}
    & \rpgbin{}     & 7.61 & 7.18 & 50.26$^\ast$ & \textbf{0.99} \\
    & \rpgboxes{}   & 9.46 & 8.84 & 170.36$^\ast$ & \textbf{1.83} \\ 
    & \rpgdesk{}    & 7.25 & 32.46 & 8.25 & \textbf{1.87} \\
    & \rpgmonitor{} & 2.74 & 7.01 & 7.77 & \textbf{0.60} \\
\midrule\\[-0.6ex]
\end{tabular}
\end{adjustbox}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llccccc}
    & & ORB-SLAM & ORB-SLAM [33] & DSO [4] & DSO$^\dagger$ & EDS (\textbf{Ours})\\ %
    & \textbf{Input} & F+F & F & F & F$^\dagger$ & E+F\\ 
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Sequence}}}
    & \rpgbin{}     & \textbf{0.58} & 0.84 & 2.12 & -  & 0.99 \\
    & \rpgboxes{}   & 4.26 & 2.39 & 2.14 & -  & \textbf{1.83} \\ 
    & \rpgdesk{}    & 2.81 & 2.52 & 63.5 & \textbf{1.80} & 1.87 \\
    & \rpgmonitor{} & 3.70 & 1.77 & \textbf{0.33} & 1.54 & 0.60\\
\midrule
\end{tabular}
\end{adjustbox}
\vspace{-1ex}
\caption{\emph{Comparison with event-based 6-DOF VO methods (top) and frame-bsaed ones (bottom)} in terms of $\text{ATE}_\text{rot}$: 
Absolute Trajectory Error (RMS)~[rot:~\si{\deg}] on sequences from [49].
Same input data and methods as Tables 2 and 3 in the paper.
}
\label{tab:compare:rot:events_and_frames}
\vspace{-2ex}
\end{table}

